Simulator-free Solution of High-Dimensional Stochastic Elliptic Partial Differential Equations using Deep Neural Networks

Stochastic partial differential equations (SPDEs) are ubiquitous in engineering and computational sciences. The stochasticity arises as a consequence of uncertainty in input parameters, constitutive relations, initial/boundary conditions, etc. Because of these functional uncertainties, the stochastic parameter space is often high-dimensional, requiring hundreds, or even thousands, of parameters to describe it. This poses an insurmountable challenge to response surface modeling since the number of forward model evaluations needed to construct an accurate surrogate grows exponentially with the dimension of the uncertain parameter space; a phenomenon referred to as the \textit{curse of dimensionality}. State-of-the-art methods for high-dimensional uncertainty propagation seek to alleviate the curse of dimensionality by performing dimensionality reduction in the uncertain parameter space. However, one still needs to perform forward model evaluations that potentially carry a very high computational burden. We propose a novel methodology for high-dimensional uncertainty propagation of elliptic SPDEs which lifts the requirement for a deterministic forward solver. Our approach is as follows. We parameterize the solution of the elliptic SPDE using a deep residual network (ResNet). In a departure from the traditional squared residual (SR) based loss function for training the ResNet, we introduce a novel physics-informed loss function derived from variational principles. Specifically, our loss function is the expectation of the energy functional of the PDE over the stochastic variables. We demonstrate our solver-free approach through various examples where the elliptic SPDE is subjected to different types of high-dimensional input uncertainties. Also, we solve high-dimensional uncertainty propagation and inverse problems.

==> others.tex <==
\section{others}
\label{sec:others}


\subsection{Problem definition}
\label{sec:problemdef}

\subsection{Solution of the elliptic PDE as a minimizer of an energy functional}
\label{sec:energyfunctional}
{\color{red} 
TODO: Use this section to describe the energy functional approach to solving the elliptic PDE. 
}

\subsection{Stochastic energy functional for the elliptic SPDE}
\label{sec:stochasticenergyfunctional}
{\color{red} 
TODO: Use this section to describe stochastic analogue of the energy functional (i.e. expectation of the energy functional over uncertain parameters) and derive the objective function to be minimized to obtain the solution of the SPDE.  
}

\subsection{Structure of the surrogate model}
\label{sec:surrogatestructure}
{
\color{red}
TODO: Describe the structure of the trial solution as a combination of basis functions, how BCs are enforced etc.
}

\subsection{Deep Neural Networks (DNNs)}
\label{sec:dnns}
{
\color{red}
TODO: Provide a quick primer on DNNs. 
}


\subsubsection{Gradient computation}
\label{sec:dnngradients}
{
\color{red}
TODO: Describe how gradients of the trial solution are obtained.
}

\subsubsection{Training}
\label{sec:dnntraining}
{
\color{red}
TODO: How is the model trained? 
}

\subsection{Complete methodology}
\label{sec:fullprocedure}
{
\color{red}
TODO: Describe the full end-to-end procedure for training/validation/testing of the proposed method. 

Use $\LaTeX$ \texttt{algorithm} environment to summarize. 
}
\\
\\
{
\color{red}
\textbf{END OF METHODOLOGY SECTION}. 
}
